Sensing Resource Allocation Against Data-Poisoning Attacks in Traffic Routing

Data-poisoning attacks can disrupt the efficient operations of transportation systems by misdirecting traffic flows via falsified data. One challenge in countering these attacks is to reduce the uncertainties on the types of attacks, such as the distribution of their targets and intensities. We introduce a resource allocation method in transportation networks to detect and distinguish different types of attacks and facilitate efficient traffic routing. The idea is to first cluster different types of attacks based on the corresponding optimal routing strategies, then allocate sensing resources to a subset of network links to distinguish attacks from different clusters via lexicographical mixed-integer programming. We illustrate the application of the proposed method using the Anaheim network, a benchmark model in traffic routing that contains more than 400 nodes and 900 links.

==> experiments/scatter.tex <==
\begin{figure}
    \centering
         \begin{tikzpicture}
    \begin{axis}[xlabel={{\footnotesize \(\gamma\)}},width=0.8\columnwidth,
            height =0.6\columnwidth,
            xtick={0, 0.2, 0.4},
            ytick={1, 1.2, 1.4},
            ytick style={draw=none},
             ymajorgrids = true,
            xmajorgrids = true,
               yticklabel style = {font=\footnotesize},
            xticklabel style = {font=\footnotesize}
            ]
        % \addplot[scatter, only marks,
        %          scatter src=explicit symbolic,
        %          nodes near coords*={},]
        %  table[x=x,y=y]{experiments/data/scatter.dat};        
    \end{axis}
\end{tikzpicture}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> introduction/adam_draft.tex <==
Vehicle cybersecurity is a timely, pressing challenge.
\cite{Koscher_Czeskis_Roesner_Patel_Kohno_Checkoway_McCoy_Kantor_Anderson_Shacham_et_al._2010}
Data-poisoning attacks have become a pressing challenge in mobility systems. 
\cite{Jain_2021}
\cite{Hahn_Munir_Behzadan_2021}
\cite{European_Network_and_Information_Security_Agency_2015}
\cite{Mecheva_Kakanakov_2020}

These attacks can come from many sources, including social media 
\cite{Jamalzadeh_Barker_González_Radhakrishnan_2022}
physical-world attacks such as placing stickers to confuse onboard autonomy systems, changing road signs to cause confusion, or changing traffic signals
\cite{Eykholt_Evtimov_Fernandes_Li_Rahmati_Xiao_Prakash_Kohno_Song_2018}
\cite{Feng_Huang_Chen_Liu_Mao_2018}
\cite{Laszka_Potteiger_Vorobeychik_Amin_Koutsoukos_2016}
\cite{Chen_Yin_Feng_Mao_Liu_2018}
A determined adversary with control of traffic control systems could create congestion-on-demand 
\cite{Reilly_Martin_Payer_Bayen_2016}

% Data-poisoning attacks & transportation
%   - Set up the need.
%   - Background.

Alternative routing attacks through data manipulation are easy to accomplish, and could cause massive disruption.
\cite{La_Fontaine_Muralidhar_Clifford_Eliassi-Rad_Nita-Rotaru_2022} 
\cite{Lin_Yu_Zhang_Yang_Ge_2018}
For example, attacks on routing for Google maps.
Here is a real-world example of changing routes using falsified data 
\cite{Eryonucu_Papadimitratos_2022}

There have been many recent developments in the counter-measures against data-poisoning attacks in mobility systems. 

Many people focus on guarding against false communication in vehicle ad-hoc networks (VANETS)
\cite{Lin_Yu_Zhang_Yang_Ge_2018}
\cite{Engoulou_Bellaïche_Pierre_Quintero_2014}
\cite{Mecheva_Kakanakov_2020}
or in federated learning scenarios 
\cite{Tolpegin_Truex_Gursoy_Liu_2020}
data spoofing attacks have been shown to be effective, even using a single attack vehicle 
\cite{Chen_Yin_Feng_Mao_Liu_2018}

% However, ____
%   - (closely-related)
However, the existing results on countering data-poisoning attacks still have many limitations. 

several works identifying worst-case attacks and countermeasures using a game-theoretic approach
\cite{Eghtesad_Li_Vorobeychik_Laszka_2023}
\cite{Halabi_Wahab_Zulkernine_2020}
While many people seek optimal, worst-case disruptions, it can be shown that finding worst-case attacks is computationally difficult
\cite{Laszka_Potteiger_Vorobeychik_Amin_Koutsoukos_2016}
In addition, targeted attacks in particular regions of the city (the business district of Chicago, for instance) can have far-reaching effects far from the center of the disruption.
\cite{Waniek_Raman_AlShebli_Peng_Rahwan_2021}

a real-world experiment that demonstrates manipulation of traffic lights, 
\cite{Ghena_Beyer_Hillaker_Pevarnek_Halderman_2014}
exploiting security flaws in 
takeaway being that small-scale attacks can have an outsized impact and be difficult to detect 
